AnyCharV: Bootstrap Controllable Character Video Generation with Fine-to-Coarse Guidance

Character video generation is a significant real-world application focused on producing high-quality videos featuring specific characters. Recent advancements have introduced various control signals to animate static characters, successfully enhancing control over the generation process. However, these methods often lack flexibility, limiting their applicability and making it challenging for users to synthesize a source character into a desired target scene. To address this issue, we propose a novel framework, AnyCharV, that flexibly generates character videos using arbitrary source characters and target scenes, guided by pose information. Our approach involves a two-stage training process. In the first stage, we develop a base model capable of integrating the source character with the target scene using pose guidance. The second stage further bootstraps controllable generation through a self-boosting mechanism, where we use the generated video in the first stage and replace the fine mask with the coarse one, enabling training outcomes with better preservation of character details. Extensive experimental results demonstrate the superiority of our method compared with previous state-of-the-art methods.

==> sections/impact.tex <==
\section*{Impact Statement}

% Directly replacing a character in a given target video is a crucial task in practice.
% Existed open-sourced works suffer from poor spatial and temporal information modeling.
% Our model significantly improve the generation performance with better identity preservation, motion smoothness, and human-object interaction.
% We believe our work will benefit various applications, such as art creation and film production.
% Although our method achieves remarkable success, it may fall short in modeling the back of a character and the reflection of a character in a mirror.
% Please be careful when using our model, especially facing these challenging scenarios.

Directly replacing a character in a given target video is a crucial task in practice. Existing open-source solutions often struggle with poor spatial and temporal information modeling. Our model significantly improves generation performance by better preserving identity, ensuring smoother motion, and enhancing human-object interaction. We believe our work will benefit various applications, such as art creation and film production.
While our method achieves remarkable success, it may fall short in modeling the back of a character from a front-facing reference image. Please exercise caution when using our model, especially in such a challenging scenario.

